The Effect of Antitrust Enforcement on Venture Capital Investments

This paper studies the effect of antitrust enforcement on venture capital (VC) investments and VC-backed companies. To establish causality, I exploit the DOJ's decision to close several antitrust field offices in 2013, which reduced the antitrust enforcement in areas near the closed offices. I find that the reduction in antitrust enforcement causes a significant decrease in VC investments in startups located in the affected areas. Furthermore, these affected VC-backed startups exhibit a reduced likelihood of successful exits and diminished innovation performance. These negative results are mainly driven by startups in concentrated industries, where incumbents tend to engage in anticompetitive behaviors more frequently. To mitigate the adverse effect, startups should innovate more to differentiate their products. This paper sheds light on the importance of local antitrust enforcement in fostering competition and innovation.

==> PaperTables_231102/vc_exit.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{The Effect of DOJ Antitrust Office Closure on VC Exits}
\label{table:vc_exit}
\begin{tabular}{l*{3}{c}}
\hline\hline
            
            &\multicolumn{1}{c}{Success}&\multicolumn{1}{c}{Acquisition}&\multicolumn{1}{c}{IPO}\\
            \cmidrule{2-4}
            &        OLS         &      OLS        &        OLS     \\
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
$\Delta Distance_{i} \times Post_t$ &      -0.002\sym{***}&      -0.001         &      -0.001\sym{***}\\
            &     (0.001)         &     (0.001)         &     (0.000)         \\
% \_cons      &       0.042\sym{***}&       0.034\sym{***}&       0.008\sym{***}\\
%             &     (0.001)         &     (0.001)         &     (0.000)         \\
\hline
Startup FE & Y & Y & Y \\
Year FE & Y & Y & Y \\
\hline
$R^2$          &       0.401         &       0.395         &       0.366         \\
Number of Obs.   &   92630         &   92630         &   92630         \\
\hline\hline
\end{tabular}
\end{table}


==> PaperTables_231102/vc_inves.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{The Effect of DOJ Antitrust Office Closures on VC Investments}
\label{table:vc_inves}
\begin{tabular}{l*{4}{c}}
\hline\hline
            
            &\multicolumn{1}{c}{Total Amount}&\multicolumn{1}{c}{Total Amount}&\multicolumn{1}{c}{Amount }&\multicolumn{1}{c}{Num of Investors}\\
            &\multicolumn{1}{c}{(Thousand \$)}&\multicolumn{1}{c}{(Thousand \$)}&\multicolumn{1}{c}{per Investor}&\multicolumn{1}{c}{per Round}\\
            \cmidrule{2-5}
            &        OLS         &        Poisson         &        Poisson &        Poisson    \\
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\

\hline
$\Delta Distance_{i} \times Post_t$ &    -332.330\sym{**} &      -0.027\sym{***}&      -0.017\sym{*}  &      -0.012\sym{*}  \\
            &   (147.229)         &     (0.011)         &     (0.010)         &     (0.007)         \\
% \_cons      &    3562.490\sym{***}&       8.678\sym{***}&       7.533\sym{***}&       0.177\sym{***}\\
%             &   (116.630)         &     (0.006)         &     (0.006)         &     (0.004)         \\
\hline
Startup FE & Y & Y & Y & Y \\
Year FE & Y & Y & Y & Y \\
\hline
$R^2$       &       0.151         &      0.407         &        0.358        &       0.220              \\
Num of Obs.     &   80211         &   80211         &   80211         &   80211         \\
\hline\hline
\end{tabular}
\end{table}


==> PaperTables_231102/vc_inves_hhi.tex <==
\begin{table}[htbp]\centering
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Mechanism: Product Market Anticompetitive Conduct by Incumbents in Concentrated Industries}
\label{table:vc_inves_hhi}
\begin{tabular}{l*{8}{c}}
\hline\hline
            &\multicolumn{2}{c}{Total Amount} &\multicolumn{2}{c}{Total Amount}&\multicolumn{2}{c}{Amount}&\multicolumn{2}{c}{Num of investors}\\
            &\multicolumn{2}{c}{(Thousand \$)} &\multicolumn{2}{c}{(Thousand \$)}&\multicolumn{2}{c}{per Investor}&\multicolumn{2}{c}{per Round}\\
            &\multicolumn{2}{c}{OLS} &\multicolumn{2}{c}{Poisson}&\multicolumn{2}{c}{Poisson}&\multicolumn{2}{c}{Poisson}\\
\cmidrule{2-9}
Industry Concentration    &    High    &    Low    &    High    &    Low    &   High    &    Low   &   High    &    Low  \\
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\

\hline
$\Delta Distance_{i} \times Post_t$ &    -269.707\sym{***}&      74.397         &      -0.040\sym{***}&       0.016         &      -0.030\sym{**} &       0.031         &      -0.029\sym{***}&       0.016         \\
            &    (88.494)         &    (91.164)         &     (0.013)         &     (0.025)         &     (0.013)         &     (0.023)         &     (0.009)         &     (0.017)         \\
% \_cons      &    3689.778\sym{***}&    3085.868\sym{***}&       8.733\sym{***}&       8.697\sym{***}&       7.579\sym{***}&       7.531\sym{***}&       0.201\sym{***}&       0.279\sym{***}\\
%             &    (73.510)         &    (69.333)         &     (0.008)         &     (0.011)         &     (0.008)         &     (0.012)         &     (0.005)         &     (0.007)         \\
\hline
Startup FE & Y & Y & Y & Y & Y & Y & Y & Y \\
Year FE & Y & Y & Y & Y & Y & Y & Y & Y \\
\hline
$R^2$       &       0.232         &       0.231         &       0.408       &       0.408        &      0.354         &       0.370        &      0.210        &       0.255         \\
Num of Obs.       &   44640         &   15374         &   44640        &   15374        &   44640         &   15374         &   44640      &   15374        \\
\hline\hline
\end{tabular}
\end{table}


==> PaperTables_231102/vc_inves_hhi_triple_diff.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Mechanism: Industry Concentration}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{Total Amount (OLS)}&\multicolumn{1}{c}{Total Amount (OLS)}&\multicolumn{1}{c}{Total Amount (Poisson)}&\multicolumn{1}{c}{Total Amount (Poisson)}\\
            &        b/se         &        b/se         &        b/se         &        b/se         \\
\hline
0.h\_hhi#c.ltreat\_intensityXpost&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.h\_hhi#c.ltreat\_intensityXpost&    -339.349\sym{***}&      -0.053\sym{*}  &      -0.060\sym{**} &      -0.043\sym{**} \\
            &   (127.081)         &     (0.029)         &     (0.027)         &     (0.019)         \\
ltreat\_intensityXpost&      71.319         &       0.014         &       0.030         &       0.015         \\
            &    (91.032)         &     (0.026)         &     (0.024)         &     (0.017)         \\
0.post#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.post#1.h\_hhi&   -3041.532\sym{***}&      -0.652\sym{***}&      -0.587\sym{***}&      -0.508\sym{***}\\
            &   (465.789)         &     (0.068)         &     (0.067)         &     (0.053)         \\
1.post#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.post#1.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
\_cons      &    4533.951\sym{***}&       8.891\sym{***}&       7.731\sym{***}&       0.393\sym{***}\\
            &   (180.885)         &     (0.019)         &     (0.020)         &     (0.019)         \\
\hline
r2          &       0.232         &                     &                     &                     \\
N           &   60014.000         &   60014.000         &   60014.000         &   60014.000         \\
\hline\hline
\end{tabular}
\end{table}


==> PaperTables_231102/vc_inves_innovative.tex <==
\begin{table}[htbp]\centering
\scriptsize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Mechanism: Potential to be a Future Monopolist}
\label{table:vc_inves_innovative}
\begin{tabular}{l*{8}{c}}
\hline\hline
            &\multicolumn{2}{c}{Total Amount} &\multicolumn{2}{c}{Total Amount}&\multicolumn{2}{c}{Amount}&\multicolumn{2}{c}{Num of investors}\\
            &\multicolumn{2}{c}{(Thousand \$)} &\multicolumn{2}{c}{(Thousand \$)}&\multicolumn{2}{c}{per Investor}&\multicolumn{2}{c}{per Round}\\
            &\multicolumn{2}{c}{OLS} &\multicolumn{2}{c}{Poisson}&\multicolumn{2}{c}{Poisson}&\multicolumn{2}{c}{Poisson}\\
\cmidrule{2-9}
Average num of patents    &    High    &    Low    &    High    &    Low    &   High    &    Low   &   High    &    Low  \\
per year pre-event            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}&\multicolumn{1}{c}{(8)}\\
\hline
$\Delta Distance_{i} \times Post_t$ &    -168.341         &    -369.598\sym{**} &      -0.016         &      -0.036\sym{***}&       0.010         &      -0.031\sym{**} &      -0.013         &      -0.011         \\
            &   (201.773)         &   (177.997)         &     (0.018)         &     (0.013)         &     (0.017)         &     (0.012)         &     (0.013)         &     (0.009)         \\

\hline
Startup FE & Y & Y & Y & Y & Y & Y & Y & Y \\
Year FE & Y & Y & Y & Y & Y & Y & Y & Y \\
\hline
$R^2$       &       0.220         &       0.126         &       0.348        &       0.419        &      0.310        &      0.367       &        0.209      &   0.216          \\
Num of Obs.      &   19036         &   61175         &   19036         &   61175         &   19036        &   61175        &   19036      &   61175      \\
\hline\hline
\end{tabular}
\end{table}


==> PaperTables_231102/vc_inves_parallel.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Parallel Trend Tests: Dynamic Effect of DOJ Antitrust Office Closures on VC Investments}
\label{table:vc_inves_parallel}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{Total Amount}&\multicolumn{1}{c}{Total Amount}&\multicolumn{1}{c}{Amount }&\multicolumn{1}{c}{Num of Investors}\\
            &\multicolumn{1}{c}{(Thousand \$)}&\multicolumn{1}{c}{(Thousand \$)}&\multicolumn{1}{c}{per Investor}&\multicolumn{1}{c}{per Round}\\
            \cmidrule{2-5}
            &        OLS         &        Poisson         &        Poisson &        Poisson    \\
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\

\hline
Before-5 &     845.143         &       0.023         &       0.029         &       0.006         \\
            &   (929.327)         &     (0.019)         &     (0.030)         &     (0.014)         \\
Before-4 &      12.758         &       0.003         &       0.013         &       0.007         \\
            &    (61.412)         &     (0.020)         &     (0.033)         &     (0.014)         \\
Before-3 &     -12.641         &       0.008         &       0.011         &       0.014         \\
            &    (56.303)         &     (0.018)         &     (0.030)         &     (0.013)         \\
Before-2 &     -46.292         &      -0.001         &       0.011         &      -0.013         \\
            &    (47.044)         &     (0.017)         &     (0.031)         &     (0.012)         \\

Current &      -8.857         &      -0.001         &       0.009         &      -0.001         \\
            &    (65.288)         &     (0.017)         &     (0.028)         &     (0.012)         \\
After+1 &    -358.483\sym{***}&      -0.027         &      -0.025         &      -0.006         \\
            &   (120.222)         &     (0.017)         &     (0.028)         &     (0.012)         \\
After+2 &    -456.427\sym{***}&      -0.024         &      -0.008         &      -0.022\sym{*}  \\
            &   (125.781)         &     (0.018)         &     (0.029)         &     (0.013)         \\
After+3 &    -112.563         &      -0.011         &      -0.013         &      -0.007         \\
            &   (106.082)         &     (0.020)         &     (0.031)         &     (0.016)         \\
After+4 &    -239.131\sym{***}&      -0.025         &      -0.030         &      -0.028         \\
            &    (88.633)         &     (0.022)         &     (0.033)         &     (0.018)         \\
% \_cons      &    3370.269\sym{***}&       8.489\sym{***}&       7.634\sym{***}&       0.175\sym{***}\\
%             &   (114.820)         &     (0.013)         &     (0.027)         &     (0.010)         \\
\hline
Startup FE & Y & Y & Y & Y \\
Year FE & Y & Y & Y & Y \\
\hline
$R^2$       &       0.150         &   0.394            &     0.371       &      0.220         \\
Num of Obs.     &   80211         &   80211         &   80211         &   80211         \\
\hline\hline
\end{tabular}
\end{table}


==> PaperTables_231102/vc_numpat.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{The Effect of DOJ Antitrust Office Closures on the Innovation of VC-Backed Startups}
\label{table:vc_numpat}
\begin{tabular}{l*{5}{c}}

\hline\hline
            &\multicolumn{1}{c}{ Patents\_t}&\multicolumn{1}{c}{Patents\_t+1}&\multicolumn{1}{c}{Patents\_t+2}&\multicolumn{1}{c}{Patents\_t+3}&\multicolumn{1}{c}{Patents\_t+4}\\
            \cmidrule{2-6}
            &        Poisson         &        Poisson         &        Poisson &        Poisson   &        Poisson  \\
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}\\ 
\hline
$\Delta Distance_{i} \times Post_t$ &      -0.032\sym{**} &      -0.025\sym{*}  &      -0.022         &      -0.024\sym{*}  &      -0.034\sym{**} \\
            &     (0.014)         &     (0.014)         &     (0.014)         &     (0.014)         &     (0.015)         \\
% \_cons      &       0.974\sym{***}&       1.034\sym{***}&       1.108\sym{***}&       1.185\sym{***}&       1.260\sym{***}\\
%             &     (0.008)         &     (0.007)         &     (0.007)         &     (0.006)         &     (0.005)         \\
\hline
Startup FE & Y & Y & Y & Y & Y \\
Year FE & Y & Y & Y & Y & Y \\
\hline
$R^2$  & 0.425  & 0.438   &  0.452   & 0.467 &  0.481 \\
Num of Obs.      &   37573         &   33284        &   28582        &   24065        &   19641       \\
\hline\hline
\end{tabular}
\end{table}


==> PaperTables_231216/vc_exit_panel.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{The Effect of DOJ Antitrust Office Closures on VC Exits}
\label{table:vc_exit}
\begin{tabular}{l*{3}{c}}
\hline\hline
            
            &\multicolumn{1}{c}{Success}&\multicolumn{1}{c}{Acquisition}&\multicolumn{1}{c}{IPO}\\
            \cmidrule{2-4}
            &        OLS         &      OLS        &        OLS     \\
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
\hline
$Treat_i \times Post_t$  &      -0.016\sym{***}&      -0.010\sym{**} &      -0.006\sym{***}\\
            &     (0.004)         &     (0.004)         &     (0.002)         \\
% \_cons      &       0.042\sym{***}&       0.034\sym{***}&       0.008\sym{***}\\
%             &     (0.001)         &     (0.001)         &     (0.000)         \\
\hline
Startup FE & Y & Y & Y \\
Year FE & Y & Y & Y \\
\hline
$R^2$        &       0.401         &       0.395         &       0.366         \\
Number of Obs.     &   92630         &   92630         &   92630        \\
\hline\hline
\end{tabular}

\vspace{1ex}
{\footnotesize \raggedright \textit{Notes.} This table reports the OLS regression results of the startup-year level model: $Y_{it} = \alpha + \beta Treat_{i} \times Post_t + \theta_i + \gamma_t + \epsilon_{it}$, where $Treat_i$ is a dummy variable equal to 1 if startup $i$ becomes farther away from antitrust field offices after office closures in 2013 and $Post_t$ indicates years after antitrust field office closures in 2013. In column (1), the dependent variable is a dummy variable equal to 1 if startup $i$ has successfully exited in year $t$, and 0 otherwise. In column (2), the dependent variable is a dummy variable equal to 1 if startup $i$ has exited by acquisition in year $t$. In column (3), the dependent variable is a dummy variable equal to 1 if startup $i$ has exited by IPO in year $t$. Startup fixed effects and year fixed effects are included in all regressions. Standard errors are clustered by startup and are reported in parentheses below the coefficient estimates. *, **, and *** denote significance at the 10\%, 5\%, and 1\% levels, respectively. \par}
\end{table}


==> PaperTables_231216/vc_inves_hhi_triple_diff.tex <==
\begin{table}[htbp]\centering
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\caption{Mechanism: Industry Concentration}
\begin{tabular}{l*{4}{c}}
\hline\hline
            &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
            &\multicolumn{1}{c}{Total Amount (OLS)}&\multicolumn{1}{c}{Total Amount (Poisson)}&\multicolumn{1}{c}{Num of investors per round}&\multicolumn{1}{c}{Amount per Investor}\\
            &        b/se         &        b/se         &        b/se         &        b/se         \\
\hline
0.treat     &       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat     &       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.post      &       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.post      &       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.treat#0.post&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.treat#1.post&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat#0.post&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat#1.post&     361.822         &       0.067         &       0.074         &       0.162         \\
            &   (312.170)         &     (0.149)         &     (0.093)         &     (0.127)         \\
0.h\_hhi     &       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.h\_hhi     &       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.treat#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.treat#1.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat#1.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.post#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.post#1.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.post#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.post#1.h\_hhi&    2180.507\sym{***}&       0.693\sym{***}&       0.514\sym{***}&       0.590\sym{***}\\
            &   (238.457)         &     (0.075)         &     (0.054)         &     (0.067)         \\
0.treat#0.post#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.treat#0.post#1.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.treat#1.post#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
0.treat#1.post#1.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat#0.post#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat#0.post#1.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat#1.post#0.h\_hhi&       0.000         &       0.000         &       0.000         &       0.000         \\
            &         (.)         &         (.)         &         (.)         &         (.)         \\
1.treat#1.post#1.h\_hhi&   -1530.249\sym{***}&      -0.315\sym{*}  &      -0.256\sym{**} &      -0.334\sym{**} \\
            &   (358.006)         &     (0.168)         &     (0.105)         &     (0.145)         \\
\_cons      &    2101.135\sym{***}&       8.510\sym{***}&       0.017         &       7.289\sym{***}\\
            &   (100.154)         &     (0.038)         &     (0.022)         &     (0.032)         \\
\hline
r2          &       0.254         &                     &                     &                     \\
N           &   60014.000         &   60014.000         &   60014.000         &   60014.000         \\
\hline\hline
\end{tabular}
\end{table}

